AirIO: Learning Inertial Odometry with Enhanced IMU Feature Observability

Inertial odometry (IO) using only Inertial Measurement Units (IMUs) offers a lightweight and cost-effective solution for Unmanned Aerial Vehicle (UAV) applications, yet existing learning-based IO models often fail to generalize to UAVs due to the highly dynamic and non-linear-flight patterns that differ from pedestrian motion. In this work, we identify that the conventional practice of transforming raw IMU data to global coordinates undermines the observability of critical kinematic information in UAVs. By preserving the body-frame representation, our method achieves substantial performance improvements, with a 66.7% average increase in accuracy across three datasets. Furthermore, explicitly encoding attitude information into the motion network results in an additional 23.8% improvement over prior results. Combined with a data-driven IMU correction model (AirIMU) and an uncertainty-aware Extended Kalman Filter (EKF), our approach ensures robust state estimation under aggressive UAV maneuvers without relying on external sensors or control inputs. Notably, our method also demonstrates strong generalizability to unseen data not included in the training set, underscoring its potential for real-world UAV applications.

==> tables/openvins.tex <==
\begin{table}[!t]
    \caption{The ATE (Unit: \meter) and RTE (Unit: \meter) on EuRoC dataset.}
    \label{euroc}
    \centering
\resizebox{0.6\linewidth}{!}{
    \begin{tabular}{C{2.3cm}|C{.8cm}C{.8cm}|C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}}
        \toprule
        \multirow{2}{*}{\textbf{Seq.}} & \multicolumn{2}{c}{\textbf{OpenVINS}$^\S$ \cite{peng2024quantized}}& \multicolumn{2}{c}{\textbf{RoNIN}$^\dagger$} & \multicolumn{2}{c}{\textbf{TLIO}$^\dagger$} & \multicolumn{2}{c}{\textbf{AirIO Net}} & \multicolumn{2}{c}{\textbf{AirIO EKF}}\\
         &  ATE  &  RTE &  ATE  &  RTE &  ATE  &  RTE &  ATE  &  RTE &  ATE  &  RTE\\
        


    \end{tabular} 
    }
\end{table}


==> tables/openvins_blackbird.tex <==
\begin{table*}[h]
    \caption{The ATE (Unit: \meter) and RTE (Unit: \meter) on the Blackbird dataset and the EuRoC dataset. \textbf{Seen} are sequences where the training and testing datasets are derived from the same trajectory.}
    \label{openvins}
    \centering
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{C{2.5cm}|C{.8cm}C{.8cm}|C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}}
        \toprule
       \multirow{2}{*}{\textbf{Seq.}} & \multicolumn{2}{c}{\textbf{OpenVINS$^\S$}~\cite{geneva2020openvins}}&   \multicolumn{2}{c}{\textbf{TLIO$^\dagger$}} & \multicolumn{2}{c}{\textbf{IMO$^\dagger$$^\ast$ }} & \multicolumn{2}{c}{\textbf{AirIO Net}} & \multicolumn{2}{c}{\textbf{AirIO EKF}}\\
         &  RTE&  ATE  &  RTE &  ATE  &  RTE &  ATE  &  RTE &  ATE  &  RTE &  ATE \\
        \midrule
        \raggedright \textbf{EuRoC} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} &\\
         MH02 &  - &\cellcolor{g1!100} \textbf{0.9} & \cellcolor{g5!100} 2.121 & \cellcolor{g5!100} 5.902 & \cellcolor{g7!100} 2.451 & \cellcolor{g7!100} 7.281 & \cellcolor{g1!100} \textbf{0.936} & \cellcolor{g3!100} 4.917 & \cellcolor{g3!100} 0.987 & \cellcolor{g2!100} 2.478 \\
         
         MH04 &-&\cellcolor{g1!100} \textbf{1.36} & \cellcolor{g5!100} 4.542 & \cellcolor{g5!100} 8.586 & \cellcolor{g7!100} 5.498 & \cellcolor{g7!100} 8.626 & \cellcolor{g3!100} 1.093 & \cellcolor{g3!100} 2.726 & \cellcolor{g1!100} \textbf{1.005} & \cellcolor{g2!100} 2.308\\

         
         V103 &
 - &\cellcolor{g1!100} \textbf{1.68} & \cellcolor{g5!100} 1.695 & \cellcolor{g3!100} 3.24 & \cellcolor{g7!100} 2.58 & \cellcolor{g7!100} 7.863 & \cellcolor{g1!100} \textbf{1.519} & \cellcolor{g5!100} 3.844 & \cellcolor{g3!100} 1.552 & \cellcolor{g2!100} 3.05 \\

         
         V202 & - &\cellcolor{g1!100} \textbf{1.24} & \cellcolor{g5!100} 2.303 & \cellcolor{g7!100} 7.445 & \cellcolor{g7!100} 2.783 & \cellcolor{g5!100} 6.26 & \cellcolor{g1!100} \textbf{1.303} & \cellcolor{g3!100} 4.823 & \cellcolor{g3!100} 1.313 & \cellcolor{g2!100} 4.206 \\
         
         V101 & - &\cellcolor{g1!100} \textbf{0.53} & \cellcolor{g5!100} 1.918 & \cellcolor{g7!100} 8.576 & \cellcolor{g7!100} 1.946 & \cellcolor{g5!100} 4.814 & \cellcolor{g3!100} 1.137 & \cellcolor{g2!100} 2.917 & \cellcolor{g1!100} \textbf{1.103} & \cellcolor{g3!100} 3.844 \\
        \midrule
        \textbf{Avg.} & - &\cellcolor{g1!100} \textbf{1.14} & \cellcolor{g5!100} 2.516 & \cellcolor{g5!100} 6.75 & \cellcolor{g7!100} 3.052 & \cellcolor{g7!100} 6.969 & \cellcolor{g3!100} 1.198 & \cellcolor{g3!100} 3.846 & \cellcolor{g1!100} \textbf{1.192} &\cellcolor{g2!100} 3.177\\
 
        \midrule
        \midrule
        \raggedright \textbf{BlackBird Seen} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} &\\
        
        \raggedright\hspace{0.3cm} Clover &- & \cellcolor{g5!100} 0.5 & \cellcolor{g7!100} 0.797 & \cellcolor{g7!100} 1.464 & \cellcolor{g5!100} 0.681 & \cellcolor{g2!100} 0.381 & \cellcolor{g1!100} \textbf{0.368} & \cellcolor{g3!100} 0.434 & \cellcolor{g3!100} 0.391 & \cellcolor{g1!100} \textbf{0.367} \\
 
        \raggedright\hspace{0.3cm} Egg &- & \cellcolor{g3!100} 1.07 & \cellcolor{g7!100} 2.398 & \cellcolor{g7!100} 2.227 & \cellcolor{g5!100} 0.828 & \cellcolor{g5!100} 1.153 & \cellcolor{g3!100} 0.391 & \cellcolor{g2!100} 0.713 & \cellcolor{g1!100} \textbf{0.344} & \cellcolor{g1!100} \textbf{0.408} \\
 

        \raggedright\hspace{0.3cm} halfMoon &-& \cellcolor{g1!100} \textbf{0.37} & \cellcolor{g7!100} 0.475 & \cellcolor{g7!100} 0.956 & \cellcolor{g1!100} \textbf{0.24} & \cellcolor{g5!100} 0.761 & \cellcolor{g5!100} 0.256 & \cellcolor{g3!100} 0.491 & \cellcolor{g3!100} 0.253 & \cellcolor{g2!100} 0.457 \\
        
        \raggedright\hspace{0.3cm} Star &- & \cellcolor{g7!100} 2.78 & \cellcolor{g5!100} 0.784 & \cellcolor{g3!100} 0.68 & \cellcolor{g7!100} 3.066 & \cellcolor{g5!100} 2.13 & \cellcolor{g3!100} 0.401 & \cellcolor{g1!100} \textbf{0.442} & \cellcolor{g1!100} \textbf{0.341} & \cellcolor{g2!100} 0.477 \\
        
        \raggedright\hspace{0.3cm} Winter &-& \cellcolor{g1!100} \textbf{0.12} & \cellcolor{g7!100} 0.755 & \cellcolor{g7!100} 0.616 & \cellcolor{g5!100} 0.206 & \cellcolor{g2!100} 0.219 & \cellcolor{g1!100} \textbf{0.147} & \cellcolor{g5!100} 0.348 & \cellcolor{g3!100} 0.164 & \cellcolor{g3!100} 0.307 \\
        \midrule
        \textbf{Avg.} & 
- & \cellcolor{g5!100} 0.97 & \cellcolor{g7!100} 1.042 & \cellcolor{g7!100} 1.189 & \cellcolor{g5!100} 1.004 & \cellcolor{g3!100} 0.929 & \cellcolor{g3!100} 0.312 & \cellcolor{g2!100} 0.486 & \cellcolor{g1!100} \textbf{0.299} & \cellcolor{g1!100} \textbf{0.403} \\
    
        \bottomrule
        \multicolumn{9}{l}{$^\dagger$ Leverage ground truth orientation to transform the input data for inference.}\\
        \multicolumn{9}{l}{$^\S$ Visual-Inertial Odometry (VIO) method.}\\
    \end{tabular} 
    }
\end{table*}


 


 

 



==> tables/transformer_architecture.tex <==
\begin{table}[h]
\centering
\begin{minipage}{0.48\linewidth}
    \caption{Comparison of Transformer-based methods on EuRoC dataset and BlackBIrd dataset. Evaluation metric: ATE (Unit: \meter) and RTE (Unit: \meter)}
    \label{euroc}
    \centering
\resizebox{0.5\linewidth}{!}{
    \begin{tabular}{C{2cm}|C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}C{.8cm}}
        \toprule
        \multirow{2}{*}
        {\textbf{Seq.}}&  \multicolumn{2}{c}{\multirow{2}{*}{\shortstack{\textbf{Transformer} \\ \textbf{$+$Global}}}} &  \multicolumn{2}{c}{\multirow{2}{*}{\shortstack{\textbf{Transformer} \\ \textbf{$+$Body}}}} &  \multicolumn{2}{c}{\multirow{2}{*}{\shortstack{\textbf{Transformer} \\ \textbf{$+$Attitude}}}} &  \multicolumn{2}{c}{\multirow{2}{*}{\textbf{AirIO Net}}}\\ 
        & & & & & &&&\\
        &  ATE  &  RTE &  ATE  &  RTE &  ATE  &  RTE &  ATE  &  RTE\\
        \midrule
        \raggedright \textbf{EuRoC}  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}\\

         MH02 &\cellcolor{g7!100} 12.03 & \cellcolor{g7!100} 2.995 & \cellcolor{g5!100} 3.357 & \cellcolor{g5!100} 1.081 & \cellcolor{g1!100} \textbf{2.452} & \cellcolor{g1!100}\textbf{0.885} & \cellcolor{g3!100} 2.531 & \cellcolor{g3!100} 0.972 \\
         
         MH04 &\cellcolor{g7!100} 11.964 & \cellcolor{g7!100} 7.395 & \cellcolor{g5!100} 4.764 & \cellcolor{g5!100} 1.159 & \cellcolor{g3!100} 2.306 & \cellcolor{g3!100} 1.096 & \cellcolor{g1!100} \textbf{2.25} & \cellcolor{g1!100} \textbf{1.009} \\

         
         V103 & \cellcolor{g7!100} 9.93 & \cellcolor{g7!100} 2.932 & \cellcolor{g5!100} 7.624 & \cellcolor{g3!100} 1.46 & \cellcolor{g3!100} 4.978 & \cellcolor{g1!100} \textbf{1.445} & \cellcolor{g1!100} \textbf{3.107} & \cellcolor{g5!100} 1.512 \\


         
         V202 &\cellcolor{g7!100} 10.689 & \cellcolor{g7!100} 3.057 & \cellcolor{g1!100} \textbf{2.521} & \cellcolor{g1!100} \textbf{1.042} & \cellcolor{g5!100} 5.567 & \cellcolor{g3!100} 1.23 & \cellcolor{g3!100} 4.31 & \cellcolor{g5!100} 1.263 \\

         V101 &\cellcolor{g5!100} 10.322 & \cellcolor{g7!100} 2.276 & \cellcolor{g7!100} 15.762 & \cellcolor{g5!100} 1.472 & \cellcolor{g3!100} 6.673 & \cellcolor{g3!100} 1.303 & \cellcolor{g1!100} \textbf{4.287} & \cellcolor{g1!100} \textbf{1.104} \\
        \textbf{Avg.} &\cellcolor{g7!100} 10.987 & \cellcolor{g7!100} 3.731 & \cellcolor{g5!100} 6.806 & \cellcolor{g5!100} 1.243 & \cellcolor{g3!100} 4.395 & \cellcolor{g3!100} 1.192 & \cellcolor{g1!100} \textbf{3.297} & \cellcolor{g1!100} \textbf{1.172} \\

        \midrule
        \midrule
    \raggedright \textbf{BB. Seen}  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}\\

    clover &\cellcolor{g7!100} 0.983 & \cellcolor{g7!100} 0.714 & \cellcolor{g3!100} 0.481 & \cellcolor{g3!100} 0.379 & \cellcolor{g5!100} 0.645 & \cellcolor{g5!100} 0.389 & \cellcolor{g1!100} \textbf{0.411} & \cellcolor{g1!100} \textbf{0.355} \\
    
   halfMoon &\cellcolor{g7!100} 0.48 & \cellcolor{g5!100} 0.23 & \cellcolor{g3!100} 0.223 & \cellcolor{g1!100} \textbf{0.129} & \cellcolor{g1!100} \textbf{0.219} & \cellcolor{g3!100} 0.219 & \cellcolor{g5!100} 0.445 & \cellcolor{g7!100} 0.243 \\
   
 star &\cellcolor{g7!100} 1.323 & \cellcolor{g7!100} 2.053 & \cellcolor{g5!100} 0.955 & \cellcolor{g5!100} 0.586 & \cellcolor{g1!100} \textbf{0.401} & \cellcolor{g3!100} 0.469 & \cellcolor{g3!100} 0.43 & \cellcolor{g1!100} \textbf{0.346} \\
 
egg&\cellcolor{g3!100} 0.698 & \cellcolor{g5!100} 0.521 & \cellcolor{g5!100} 0.914 & \cellcolor{g3!100} 0.479 & \cellcolor{g7!100} 1.013 & \cellcolor{g7!100} 0.79 & \cellcolor{g1!100} \textbf{0.677} & \cellcolor{g1!100} \textbf{0.356} \\

 winter&\cellcolor{g7!100} 0.856 & \cellcolor{g7!100} 0.548 & \cellcolor{g1!100} \textbf{0.276} & \cellcolor{g3!100} 0.215 & \cellcolor{g5!100} 0.386 & \cellcolor{g5!100} 0.325 & \cellcolor{g3!100} 0.359 & \cellcolor{g1!100} \textbf{0.165} \\

\textbf{Avg.} & \cellcolor{g7!100} 0.868 & \cellcolor{g7!100} 0.813 & \cellcolor{g5!100} 0.57 & \cellcolor{g3!100} 0.358 & \cellcolor{g3!100} 0.532 & \cellcolor{g5!100} 0.438 & \cellcolor{g1!100} \textbf{0.464} & \cellcolor{g1!100} \textbf{0.293} \\
    \midrule
    \midrule
\raggedright \textbf{BB. Unseen}  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}\\
ampersand &\cellcolor{g7!100} 11.4 & \cellcolor{g7!100} 4.417 & \cellcolor{g5!100} 3.112 & \cellcolor{g5!100} 1.954 & \cellcolor{g1!100} \textbf{1.931} & \cellcolor{g3!100} 1.428 & \cellcolor{g3!100} 2.492 & \cellcolor{g1!100} \textbf{1.185} \\

 sid&\cellcolor{g7!100} 3.932 & \cellcolor{g7!100} 5.765 & \cellcolor{g5!100} 1.564 & \cellcolor{g3!100} 0.842 & \cellcolor{g3!100} 0.824 & \cellcolor{g5!100} 0.847 & \cellcolor{g1!100} \textbf{0.651} & \cellcolor{g1!100} \textbf{0.504} \\
 
oval&\cellcolor{g7!100} 8.935 & \cellcolor{g7!100} 5.137 & \cellcolor{g3!100} 0.707 & \cellcolor{g1!100} \textbf{0.463} & \cellcolor{g1!100} \textbf{0.614} & \cellcolor{g5!100} 0.639 & \cellcolor{g5!100} 0.913 & \cellcolor{g3!100} 0.558 \\
 
sphinx&\cellcolor{g7!100} 3.778 & \cellcolor{g7!100} 4.971 & \cellcolor{g5!100} 1.396 & \cellcolor{g3!100} 1.164 & \cellcolor{g1!100} \textbf{1.139} & \cellcolor{g5!100} 1.78 & \cellcolor{g3!100} 1.164 & \cellcolor{g1!100} \textbf{1.022} \\
 
bentDice&\cellcolor{g7!100} 3.904 & \cellcolor{g7!100} 3.755 & \cellcolor{g5!100} 1.594 & \cellcolor{g3!100} 1.266 & \cellcolor{g3!100} 1.437 & \cellcolor{g5!100} 1.36 & \cellcolor{g1!100} \textbf{1.249} & \cellcolor{g1!100} \textbf{0.872} \\
 
\textbf{Avg.} & \cellcolor{g7!100} 6.39 & \cellcolor{g7!100} 4.809 & \cellcolor{g5!100} 1.675 & \cellcolor{g3!100} 1.138 & \cellcolor{g1!100} \textbf{1.189} & \cellcolor{g5!100} 1.211 & \cellcolor{g3!100} 1.294 & \cellcolor{g1!100} \textbf{0.828} \\

    
        \bottomrule
        % \multicolumn{9}{l}{$^\dagger$ Leverage ground truth orientation to transform the input data for inference.}\\

    \end{tabular}
    }
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
 \centering
    \includegraphics[width=0.5\linewidth]{figs/Transformer.pdf}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{minipage}
\end{table}



==> tables/transformer_table.tex <==
\begin{table}[h]
    \caption{Comparison of Transformer-based methods on EuRoC dataset and BlackBIrd dataset. Evaluation metric: ATE (Unit: \meter) and RTE (Unit: \meter)}
    \label{transformer_ablation}
    \centering
\resizebox{0.6\linewidth}{!}{
    \begin{tabular}{C{2cm}|C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}}
        \toprule
        \multirow{2}{*}
        {\textbf{Seq.}}&  \multicolumn{2}{c}{\multirow{2}{*}{\shortstack{\textbf{Global-Frame} \\ \textbf{with Transformer}}}} &  \multicolumn{2}{c}{\multirow{2}{*}{\shortstack{\textbf{Body-Frame} \\ \textbf{with Transformer}}}} &  \multicolumn{2}{c}{\multirow{2}{*}{\shortstack{\textbf{AirIO} \\ \textbf{with Transformer}}}} &  \multicolumn{2}{c}{\multirow{2}{*}{\textbf{AirIO Net}}}\\ 
        & & & & & &&&\\
        &  ATE  &  RTE &  ATE  &  RTE &  ATE  &  RTE &  ATE  &  RTE\\
        \midrule
        \raggedright \textbf{EuRoC}  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}\\

         MH02 &\cellcolor{g7!100} 12.03 & \cellcolor{g7!100} 2.995 & \cellcolor{g5!100} 3.357 & \cellcolor{g5!100} 1.081 & \cellcolor{g1!100} \textbf{2.452} & \cellcolor{g1!100}\textbf{0.885} & \cellcolor{g3!100} 2.531 & \cellcolor{g3!100} 0.972 \\
         
         MH04 &\cellcolor{g7!100} 11.964 & \cellcolor{g7!100} 7.395 & \cellcolor{g5!100} 4.764 & \cellcolor{g5!100} 1.159 & \cellcolor{g3!100} 2.306 & \cellcolor{g3!100} 1.096 & \cellcolor{g1!100} \textbf{2.25} & \cellcolor{g1!100} \textbf{1.009} \\

         
         V103 & \cellcolor{g7!100} 9.93 & \cellcolor{g7!100} 2.932 & \cellcolor{g5!100} 7.624 & \cellcolor{g3!100} 1.46 & \cellcolor{g3!100} 4.978 & \cellcolor{g1!100} \textbf{1.445} & \cellcolor{g1!100} \textbf{3.107} & \cellcolor{g5!100} 1.512 \\


         
         V202 &\cellcolor{g7!100} 10.689 & \cellcolor{g7!100} 3.057 & \cellcolor{g1!100} \textbf{2.521} & \cellcolor{g1!100} \textbf{1.042} & \cellcolor{g5!100} 5.567 & \cellcolor{g3!100} 1.23 & \cellcolor{g3!100} 4.31 & \cellcolor{g5!100} 1.263 \\

         V101 &\cellcolor{g5!100} 10.322 & \cellcolor{g7!100} 2.276 & \cellcolor{g7!100} 15.762 & \cellcolor{g5!100} 1.472 & \cellcolor{g3!100} 6.673 & \cellcolor{g3!100} 1.303 & \cellcolor{g1!100} \textbf{4.287} & \cellcolor{g1!100} \textbf{1.104} \\
        \textbf{Avg.} &\cellcolor{g7!100} 10.987 & \cellcolor{g7!100} 3.731 & \cellcolor{g5!100} 6.806 & \cellcolor{g5!100} 1.243 & \cellcolor{g3!100} 4.395 & \cellcolor{g3!100} 1.192 & \cellcolor{g1!100} \textbf{3.297} & \cellcolor{g1!100} \textbf{1.172} \\

        \midrule
        \midrule
    \raggedright \textbf{BB. Seen}  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}\\

    clover &\cellcolor{g7!100} 0.983 & \cellcolor{g7!100} 0.714 & \cellcolor{g3!100} 0.481 & \cellcolor{g3!100} 0.379 & \cellcolor{g5!100} 0.645 & \cellcolor{g5!100} 0.389 & \cellcolor{g1!100} \textbf{0.411} & \cellcolor{g1!100} \textbf{0.355} \\
    
   halfMoon &\cellcolor{g7!100} 0.48 & \cellcolor{g5!100} 0.23 & \cellcolor{g3!100} 0.223 & \cellcolor{g1!100} \textbf{0.129} & \cellcolor{g1!100} \textbf{0.219} & \cellcolor{g3!100} 0.219 & \cellcolor{g5!100} 0.445 & \cellcolor{g7!100} 0.243 \\
   
 star &\cellcolor{g7!100} 1.323 & \cellcolor{g7!100} 2.053 & \cellcolor{g5!100} 0.955 & \cellcolor{g5!100} 0.586 & \cellcolor{g1!100} \textbf{0.401} & \cellcolor{g3!100} 0.469 & \cellcolor{g3!100} 0.43 & \cellcolor{g1!100} \textbf{0.346} \\
 
egg&\cellcolor{g3!100} 0.698 & \cellcolor{g5!100} 0.521 & \cellcolor{g5!100} 0.914 & \cellcolor{g3!100} 0.479 & \cellcolor{g7!100} 1.013 & \cellcolor{g7!100} 0.79 & \cellcolor{g1!100} \textbf{0.677} & \cellcolor{g1!100} \textbf{0.356} \\

 winter&\cellcolor{g7!100} 0.856 & \cellcolor{g7!100} 0.548 & \cellcolor{g1!100} \textbf{0.276} & \cellcolor{g3!100} 0.215 & \cellcolor{g5!100} 0.386 & \cellcolor{g5!100} 0.325 & \cellcolor{g3!100} 0.359 & \cellcolor{g1!100} \textbf{0.165} \\

\textbf{Avg.} & \cellcolor{g7!100} 0.868 & \cellcolor{g7!100} 0.813 & \cellcolor{g5!100} 0.57 & \cellcolor{g3!100} 0.358 & \cellcolor{g3!100} 0.532 & \cellcolor{g5!100} 0.438 & \cellcolor{g1!100} \textbf{0.464} & \cellcolor{g1!100} \textbf{0.293} \\
    \midrule
    \midrule
\raggedright \textbf{BB. Unseen}  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}\\
ampersand &\cellcolor{g7!100} 11.4 & \cellcolor{g7!100} 4.417 & \cellcolor{g5!100} 3.112 & \cellcolor{g5!100} 1.954 & \cellcolor{g1!100} \textbf{1.931} & \cellcolor{g3!100} 1.428 & \cellcolor{g3!100} 2.492 & \cellcolor{g1!100} \textbf{1.185} \\

 sid&\cellcolor{g7!100} 3.932 & \cellcolor{g7!100} 5.765 & \cellcolor{g5!100} 1.564 & \cellcolor{g3!100} 0.842 & \cellcolor{g3!100} 0.824 & \cellcolor{g5!100} 0.847 & \cellcolor{g1!100} \textbf{0.651} & \cellcolor{g1!100} \textbf{0.504} \\
 
oval&\cellcolor{g7!100} 8.935 & \cellcolor{g7!100} 5.137 & \cellcolor{g3!100} 0.707 & \cellcolor{g1!100} \textbf{0.463} & \cellcolor{g1!100} \textbf{0.614} & \cellcolor{g5!100} 0.639 & \cellcolor{g5!100} 0.913 & \cellcolor{g3!100} 0.558 \\
 
sphinx&\cellcolor{g7!100} 3.778 & \cellcolor{g7!100} 4.971 & \cellcolor{g5!100} 1.396 & \cellcolor{g3!100} 1.164 & \cellcolor{g1!100} \textbf{1.139} & \cellcolor{g5!100} 1.78 & \cellcolor{g3!100} 1.164 & \cellcolor{g1!100} \textbf{1.022} \\
 
bentDice&\cellcolor{g7!100} 3.904 & \cellcolor{g7!100} 3.755 & \cellcolor{g5!100} 1.594 & \cellcolor{g3!100} 1.266 & \cellcolor{g3!100} 1.437 & \cellcolor{g5!100} 1.36 & \cellcolor{g1!100} \textbf{1.249} & \cellcolor{g1!100} \textbf{0.872} \\
 
\textbf{Avg.} & \cellcolor{g7!100} 6.39 & \cellcolor{g7!100} 4.809 & \cellcolor{g5!100} 1.675 & \cellcolor{g3!100} 1.138 & \cellcolor{g1!100} \textbf{1.189} & \cellcolor{g5!100} 1.211 & \cellcolor{g3!100} 1.294 & \cellcolor{g1!100} \textbf{0.828} \\

    
        \bottomrule
        % \multicolumn{9}{l}{$^\dagger$ Leverage ground truth orientation to transform the input data for inference.}\\

    \end{tabular} 
    }
\end{table}




